Advanced transceivers for spectrally-efficient communications

In this thesis, we will consider techniques to improve the spectral efficiency of digital communication systems, operating on the whole transceiver scheme. First, we will focus on receiver schemes having detection algorithms with a complexity constraint. We will optimize the parameters of the reduced detector with the aim of maximizing the achievable information rate. Namely, we will adopt the channel shortening technique. Then, we will focus on a technique that is getting very popular in the last years (although presented for the first time in 1975): faster-than-Nyquist signaling, and its extension which is time packing. Time packing is a very simple technique that consists in introducing intersymbol interference on purpose with the aim of increasing the spectral efficiency of finite order constellations. Finally, in the last chapters we will combine all the presented techniques, and we will consider their application to satellite channels.

==> conc.tex <==
\chapter*{Conclusions}
